Differentiable Particle Filtering without Modifying the Forward Pass

Particle filters are not compatible with automatic differentiation due to the presence of discrete resampling steps. While known estimators for the score function, based on Fisher's identity, can be computed using particle filters, up to this point they required manual implementation. In this paper we show that such estimators can be computed using automatic differentiation, after introducing a simple correction to the particle weights. This correction utilizes the stop-gradient operator and does not modify the particle filter operation on the forward pass, while also being cheap and easy to compute. Surprisingly, with the same correction automatic differentiation also produces good estimators for gradients of expectations under the posterior. We can therefore regard our method as a general recipe for making particle filters differentiable. We additionally show that it produces desired estimators for second-order derivatives and how to extend it to further reduce variance at the expense of additional computation.

==> sections/0_intro.tex <==
\section{Introduction}

Particle filters \citep{doucet2009tutorial,chopin2020introduction,doucet2001introduction} are an extremely popular family of algorithms for state estimation in non-linear state space models. Their versatility, ease of implementation, and well-understood theoretical behavior make them a popular choice in a wide variety of application domains, including robotics, ecology, and finance. The crucial advantage of particle filters is that they can adaptively focus computation on more promising trajectories, which is usually accomplished through discrete resampling steps.

With the growing popularity of gradient-based end-to-end learning, particle filters have increasingly been used for model learning. Examples include robotic localization \citep{jonschkowski_differentiable_2018}, world-modeling in reinforcement learning \citep{igl2018deep}, and deep generative modeling of music and speech \citep{maddison_filtering_2017}. In such applications gradients of a particle-filter-estimated marginal likelihood objective are typically computed using backpropagation \citep{rumelhart_learning_1986}, which does not handle the discrete particle filter resampling steps correctly and introduces bias which does not vanish asymptotically \citep{corenflos_differentiable_2021}. While in principle this problem can be corrected by using score function estimators, \citet{le_auto-encoding_2018, maddison_filtering_2017, naesseth_variational_2018} all find the variance of such estimators to be too high to be practical.

Several recent articles have proposed differentiable versions of this resampling step, either relying on ideas from optimal transport and gradients arrived at via the implicit function theorem \citep{corenflos_differentiable_2021} or learned resampling networks \citep{zhan_interaction_2019}. While achieving differentiability, these algorithms significantly alter the forward pass of the particle filter, requiring large amounts of additional code, introducing additional hyperparameters that require tuning, and sometimes significantly increase the overall computational complexity. Additionally, these approaches to differentiable resampling modify the {\em values} of the particles which can lead to unexpected and potentially undesirable results.

In this work we show that it is possible to obtain unbiased gradient estimators for the marginal likelihood from a particle filter without modifying its behavior on the forward pass, and without the excess variance associated with score function estimators. We achieve this by careful use of the `stop-gradient' operator available in automatic differentiation libraries, which effectively allows us to attach auxiliary gradients to the weights in the particle filter, correcting for bias introduced by backpropagation. Our algorithm, which we call \emph{stop-gradient resampling} (SGR), requires only one simple modification to existing particle filter code, as shown in Algorithm \ref{alg:pf}. It requires no software dependencies and introduces no additional hyperparameters. It is also compatible, without any adjustments, with all of popular resampling schemes, and various flavors of nested sequential Monte Carlo \cite{naesseth_nested_2015}. Stop-gradient resampling can be regarded as an extension of the DiCE estimator \citep{foerster_dice_2018} and inherits its ability to produce unbiased estimators for higher order derivatives.



\begin{algorithm}
\caption{Forward pass of a standard particle filter. The only modification required by our algorithm, stop-gradient resampling, is highlighted in yellow. The $\bot$ denotes the stop-gradient operator, a standard component of automatic differentiation libraries. The code listing shows the corresponding modification of a typical PyTorch implementation, where stop-gradient is called detach. Where $i$ is not bounded it denotes an operation applied across all $i \in 1:N$}
\label{alg:pf}
\begin{minipage}{0.45\textwidth}
\begin{algorithmic}
\Function{PF}{$p$, $q$, $N$, $T$}
  \State $x_0^i \sim p(x_0)$
  \State $w_0^i = \normalized{w}_0^i = \frac{1}{N}$
  \For{$t \in 1:T$}
    \If{resampling condition}
      \State $a^i_{t} \sim R(\normalized{w}^{1:N}_{t-1})$
      \State $\resampled{w}^i_{t-1} = \frac{1}{N} $ \colorbox{yellow}{$\displaystyle {\normalized{w}^{a^i_{t}}_{t-1} / {\stopgrad{\normalized{w}^{a^i_t}_{t-1}}}}$}
     \Else
       \State $a^i_t = i$
       \State $\resampled{w}^i_t = \normalized{w}^{i}_{t-1}$
    \EndIf
    \State $x^i_t \sim q(x_t | x^{a_t^i}_{t-1}, y_{1:T})$
    \State $w^i_t = \resampled{w}^i_{t-1} \frac{p(x^i_t, y_t | x^{a_t^i}_{t-1})}{q(x^i_t | x^{a_t^i}_{t-1}, y_t)}$
    \State $W_t = \sum_{i=1}^N w^i_{t}$
    \State $\normalized{w}^i_t = w^i_t / W_t$
  \EndFor
  \State $Z = \prod_{t=1}^T W_t$
\EndFunction
\end{algorithmic}
\end{minipage}
\begin{minipage}{0.5\textwidth}
\begin{lstlisting}[basicstyle=\footnotesize\ttfamily, breaklines=true]
ancestral_logw = torch.gather(log_weights[-1], index=ancestral_indices[-1], dim=1)
logw += ancestral_logw - ancestral_logw.detach()
\end{lstlisting}
\end{minipage}
\end{algorithm}


==> sections/1_preliminaries.tex <==
\section{Preliminaries}

\subsection{Particle filters} \label{sec:pf}

Here we briefly review the basic particle filter algorithm, referring the reader to \citep{chopin2020introduction,doucet2009tutorial,doucet2001introduction} for more details. For a given sequence of observations $y_{1:T}$, particle filters approximate the filtering distributions $p_{\theta}(x_t | y_{1:t})$ and the marginal likelihood $p_{\theta}(y_{1:T})$ of a state space model with the following factorization of the joint
\begin{align}
    p_{\theta}(x_{0:T}, y_{1:T}) = p_{\theta}(x_0) \prod_{t=1}^T p_{\theta}(x_t | x_{t-1}) p_{\theta}(y_t | x_t).
\end{align}

The algorithm starts by sampling $N$ particles independently from the initial distribution $x_0^i \sim p_{\theta}(x_0)$ and setting their weights uniform $w_0^i = \frac{1}{N}$. Then, at each iteration it advances one step forward in time, by first advancing each particle according to the proposal distribution $q_{\theta}(x_{t+1} | x_t, y_{t+1})$, then accumulating the importance sampling ratio $\frac{p_{\theta}(x_{t+1} | x_t)}{q_{\theta}(x_{t+1} | x_t, y_{t+1})} $ and the likelihood $p_{\theta}(y_{t+1})$ in the corresponding weight, saving the sum of weights and normalizing them before proceeding to the next time step. We assume that $q$ and $p$ have the same support and that the likelihoods are always non-zero, which guarantees that all the weights are always positive. We also assume that both $p$ and $q$ are differentiable with respect to their parameters.

As the weights accumulate more terms, they become increasingly unbalanced and it is more efficient to focus more computational resources to particles with higher weights. This is accomplished via a resampling step, which in our formulation is optionally performed at the beginning of each time step. The ancestral indices for each particle are chosen from a resampling distribution $R(\normalized{w}_{t-1}^{1:N})$, which in the simplest multinomial resampling picks ancestral indices independently from a categorical distribution, but other variants like stratified and systematic resampling are usually favored in practice \citep{murray2016parallel}. Regardless of which resampling distribution is used, the weights after resampling are reset to uniform. Particle filter pseudocode is given in Algorithm \ref{alg:pf}. Note that we write $\resampled{w}$ for the weights obtained after resampling, which in a standard particle filter are always $\frac{1}{N}$, $w$ for weights after the likelihood was accumulated at a given time step, and $\normalized{w}$ for the subsequently normalized weights.

Regardless of the specific details of the particle filter algorithm used, the marginal likelihood $Z = p(y_{1:T})$ is approximated by $\hat{Z} = \prod_{t=1}^T W_t$. This estimator is known to be unbiased and under weak assumptions consistent. We refer the reader to \citet{moral_feynman-kac_2004} and \citet{chopin2020introduction} for detailed convergence results. In this paper we also use the marginal likelihood for the subsequent time steps given a current population, which we define as
\begin{align}
    F_t\left(x_t^{1:N}, \normalized{w}_t^{1:N}, \theta\right) = \sum_{i=1}^N \normalized{w}_t^i \ p_{\theta}\left(y_{t+1:T} | x_t^i\right)
\end{align}
and which satisfies the following recursive relationship
\begin{align}
    F_t\left(x_t^{1:N}, \normalized{w}_t^{1:N}, \theta\right) = \E_{a_t^i}\E_{x_{t+1}^i}\left[W_{t+1} \cdot F_{t+1}\left(x_{t+1}^{1:N}, \normalized{w}_{t+1}^{1:N}, \theta\right)\right]
\end{align}
for $a_t^i \sim R(\normalized{w}_t^{1:N})$, $x_{t+1}^i \sim q_{\theta}(x_{t+1} | x_t^{a_t^i}, y_{t+1})$.  Finally, we write $\expect{\cdot}{PF}$ for an expectation under the remaining steps of the particle filter, for example $\expect{\hat{Z}}{PF} = Z$. Additionally, $\expect{\prod_{t+1}^T W_t}{PF} = F_t(x_t^{1:N}, \normalized{w}_t^{1:N}, \theta)$, so we define $\hat{F}_t = \prod_{t+1}^T W_t$.


\subsection{Resampling with arbitrary probabilities} \label{sec:resampling}

In a particle filter it is usual to resample with probabilities proportional to weights. However, it is possible to resample with any probabilities and still obtain an unbiased estimator for the marginal likelihood, provided that all particles with non-zero weight are assigned non-zero resampling probabilities.

\begin{definition} \label{def:resampling}
Given a particle population $x^{1:N}, \normalized{w}^{1:N}$, resampling probabilities $r^{1:N}$, where $\sum_i r^i = 1$ and $r^i > 0$ for all $i$, and a resampling distribution $R$, the \emph{weighted resampling scheme} produces a random particle population $\tilde{x}^{1:N}, \tilde{w}^{1:N}$ according to the following equations:
\begin{align}
    a^i &\sim R(r^{1:N}) , \quad
    \tilde{x}^i = x^{a^i} , \quad
    \tilde{w}^i = \frac{1}{N} \frac{\normalized{w}^{a^i}}{r^{a^i}} .
\end{align}
\end{definition}

Note that when $r^{1:N} = \normalized{w}^{1:N}$, this recoveres the original resampling scheme. For any unbiased resampling scheme, such as multinomial or systematic, the associated weighted resampling scheme is also unbiased, since the resulting weights correct for using different resampling probabilities. While we were not able to find a definitive reference, this property appears to be well-understood by particle filtering practitioners. In particular, \citet{karkus_particle_2018} use it to resample using a mixture of particle weights and uniform probabilities, allowing some gradients to be backpropagated at the expense of making resampling less effective. In this work we show that it is possible to backpropagate all the necessary information, while maintaining the usual resampling behavior, by combining this observation with the stop-gradient operator.

\subsection{The stop-gradient operator} \label{sec:stop-gradient}

The stop-gradient operator is a standard component of automatic differentiation libraries, called \lstinline{stop_gradient} in Tensorflow and \lstinline{detach} in PyTorch, producing an expression that evaluates to its normal value on the forward pass but has zero gradient. While it does not correspond to any mathematical function, it provides a convenient notation to derive certain gradient estimators. Following \citet{foerster_dice_2018}, we denote the stop-gradient with a $\bot$, that is $\frac{d}{dx} \stopgrad{x} = 0$.

Such stop-gradient expressions are in particular useful for defining surrogate functions, which can be automatically differentiated to yield unbiased gradients of objectives incorporating expectations estimated with sampling. For example, DiCE \citep{foerster_dice_2018} defines a surrogate in the form of $f(x) p_{\theta}(x) / \stopgrad{p_{\theta}(x)}$, which yields correct unbiased estimators for derivatives of any order for the target $\expect{f(x)}{x \sim p_{\theta}}$. In this work we show that DiCE can be interpreted as a form of importance sampling, which naturally extends to particle filtering, allowing us to obtain unbiased derivative estimators of any order.

\subsection{Differentiable resampling} \label{sec:diff-resampling}

Backpropagating through a particle filter requires special treatment of the sampling actions, both for particle transitions and for ancestor indices, if unbiased gradient estimates are to be obtained. For the particle transitions we assume that the reparameterization trick is applicable, that is that sampling from $q_{\theta}$ can be expressed as a deterministic transformation of a random variable sampled from some standard base distribution, here assumed to be, without loss of generality, the standard normal distribution $\mathcal{N}$. Specifically, we assume there exist differentiable functions $h_t$ such that for any function $f$ we have
\begin{align}
    \expect{f(x_{t+1})}{x_{t+1} \sim q_{\theta}(x_{t+1} | x_t, y_{t+1})} = \expect{f(h_t(\epsilon_{t+1}, \theta))}{\epsilon_{t+1} \sim \mathcal{N}} ,
\end{align}
so we express the forward pass of the particle filter in terms of sampling $\epsilon$ instead of $x$, and standard backpropagation can be applied without introducing bias. Note that neither this reparameterization trick, nor typical relaxations \citep{maddison2016concrete}, can be used when sampling ancestral indices, since the resampling distribution is fundamentally discrete and directly impacts the control flow of the particle filter algorithm.

The naive way to obtain unbiased gradient estimates for the resampling steps is to use score function estimators, also called REINFORCE \citep{williams_simple_1992}, which add terms of the form $\hat{Z} \grad_{\theta} \log w^i_t$ to the biased gradient estimator obtained by automatic differentiation. Such corrections, however, are known to suffer from high variance. Specifically in the context of particle filtering, \citet{le_auto-encoding_2018, naesseth_variational_2018, maddison_filtering_2017} all report achieving better performance by ignoring such score function corrections, which we also corroborate in our experiments in Section \ref{sec:experiments}. Similarly, \citet{jonschkowski_differentiable_2018} construct an algorithm they call Differentiable Particle Filtering, which explicitly ignores the propagation of gradients through the resampling steps. They suggest adding auxiliary gradients to weights in an attempt to mitigate the resulting bias as a direction of future work. The stop-gradient resampling algorithm we present in this paper can be regarded as a concrete instantiation of this idea.

All the existing approaches that backpropagate gradients through the resampling steps also modify the resampling behavior on the forward pass, either producing non-uniform weights or introducing bias. \citet{karkus_particle_2018} use the property  we reviewed in Section \ref{sec:resampling} to resample with probabilities proportional to $\alpha w^i + \frac{1 - \alpha}{N}$, which effectively interpolates between no resampling and no gradient bias forcing the users to make an undesirable trade-off. \citet{corenflos_differentiable_2021} replace traditional resampling with a continuous transformation of particles based on optimal transport equations. This is computationally intensive, biased, and can lead to undesirable behavior, in the extreme cases even putting the resampled particles outside of the support of the prior. \citet{zhu_towards_2020} modify particles in a similar fashion using learned resampling networks, with similar disadvantages, noting that in practice propagating gradients through them leads to instabilities so they avoid it. In this work we demonstrate that it is possible to obtain unbiased gradients of the marginal likelihood from a particle filter without modifying its behavior on the forward pass at all. Unlike the methods of \citet{corenflos_differentiable_2021, zhu_towards_2020}, ours does not involve extensive implementation effort or computational cost and unlike any of the methods described in this paragraph does not introduce additional hyperparameters that need to be tuned.



==> sections/2_method.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.49\textwidth]{sections/figs/lgssm/ssm.pdf}
    \includegraphics[width=0.49\textwidth]{sections/figs/lgssm/ssm_zoomed_in.pdf}
    \caption{Estimates for the test set log-marginal likelihood throughout the training of the LGSSM model. The right plot is the zoomed in version of the left one, demonstrating the improvement of DPF-SGR over PF.}
    \label{fig:experiments/lgssm}
\end{figure}

\section{Method} \label{sec:method}

To correctly backpropagate through the resampling steps, we first interpret the DiCE estimator as a form of importance sampling. This interpretation provides a recipe for propagating the necessary corrections when constructing the computation graph, which we describe in Section \ref{sec:sgr}. Since the stop-gradient operator is convenient but not well-defined mathematically, in Section \ref{sec:theory} we rigorously define stop-gradient resampling by explicitly constructing the backward messages and prove that the resulting gradient estimators are unbiased.

\subsection{Stop-gradient resampling} \label{sec:sgr}

Our key insight is that we can derive the score function estimator, and more generally DiCE for higher order derivatives, using a form of importance sampling with the stop-gradient operator
\begin{align}
    \grad_{\theta} \E_{p_{\theta}(x)} \left[f(x)\right] = \grad_{\theta} &\E_{\stopgrad{p_{\theta}(x)}} \left[f(x) \frac{p_{\theta}(x)}{\stopgrad{p_{\theta}(x)}} \right]
      = \E_{\stopgrad{p_{\theta}(x)}} \left[f(x) \frac{\grad_{\theta} p_{\theta}(x)}{\stopgrad{p_{\theta}(x)}} \right],
\end{align}
where we drop the stop-gradient after moving the gradient inside the expectation, yielding the score function estimator
\begin{align}
    \E_{\stopgrad{p_{\theta}(x)}} \left[f(x) \frac{\grad_{\theta} p_{\theta}(x)}{\stopgrad{p_{\theta}(x)}} \right] = \E_{p_{\theta}(x)} \left[f(x) \grad_{\theta} \log  p_{\theta}(x) \right].
\end{align}

Simply changing the expectation to be with respect to the stop-gradient distribution lets us push the gradient inside without introducing bias, while the correcting factor $p_{\theta}(x) / \stopgrad{p_{\theta}(x)}$ can be regarded as an importance weight. While multiplying it with $f(x)$ yields the DiCE estimator, our key insight is that we can also use this correcting factor in a more sophisticated way, in particular to adjust particle weights {\em ex post facto}.

Specifically, we use the weighted resampling scheme from Section \ref{sec:resampling} with $r^i = \stopgrad{\normalized{w}^i}$, which corrects the resulting uniform weights with the multiplicative factor of $\normalized{w}^{a^i_t}_t / {\stopgrad{\normalized{w}^{a^i_t}_t}}$. Importantly, this ``correction'' is equal to $1$ on the forward pass, but produces auxiliary gradients on the backward pass. It therefore does not modify the behavior of the particle filter on the forward pass, and the careful use of the stop-gradient operator allows us to keep the automatic differentiation process black-box. The necessary correction, shown in Algorithm \ref{alg:pf}, requires minimal changes in implementation. We call this approach the stop-gradient resampling (SGR).

Combined with the reparameterization trick for the proposal distributions used to propagate particles through time, SGR yields a fully differentiable particle filter (DPF-SGR), where we can use automatic differentiation to obtain unbiased gradient estimators for the marginal likelihood and any expectations under the unnormalized posterior. In other words, if a particle filter provides an unbiased estimator of some quantity, DPF-SGR provides unbiased estimates for its gradients. Just like with DiCE, automatic differentiation can be applied repeatedly to obtain unbiased estimators for derivatives of higher order. DPF-SGR also automatically extends to nested particle filters \citep{naesseth_nested_2015}.

\subsection{Formal definition} \label{sec:theory}

In Section \ref{sec:sgr} we formulated our DPF-SGR algorithm using the stop-gradient operator, which is convenient but not well-defined mathematically. In this section we provide an equivalent formulation of DPF-SGR, which avoids using the stop-gradient operator by directly deriving a custom version of backpropagation for computing gradient estimators. We emphasize that this construction is not required for implementation, since the automatic differentiation libraries implementing the stop-gradient operator handle it automatically, and that we only introduce it to formally show that the gradient estimators provided by DPF-SGR are unbiased.

The majority of work in this section is straightforward application of the chain rule for computing derivatives. The only difference is in computing the backward message for the weights, which in normal backpropagation would be zero. This message is theoretically justified by applying a weighted resampling scheme and then setting resampling probabilities to equal weights after the gradient is applied, as shown in the proof of Theorem \ref{th:unbiased}.

We restrict our derivation to the univariate case, for both $x$ and $\theta$, to take advantage of the established notation for partial and total derivatives. The extension to the multivariate case is straightforward. For the purposes of calculating partial derivatives we assume the following functional relationships:
\begin{align}
    x_0 &= x_0(\theta) & x_{t+1}^i &= x_{t+1}^i \left(x_{t}^{a_t^i}, \theta\right) & w_{t}^i &= w_{t}^i\left(x_{t}^i, \theta\right) & \normalized{w}_t^i &= \normalized{w}_t^i\left(w_t^{1:N}\right).
\end{align}
\begin{definition} \label{def:gradients}
The DPF-SGR gradient is a random variable defined as $G(\theta) = \backward{\theta}_0 + \frac{1}{N} \sum_{i=1}^{N} \frac{d x_0^i}{d \theta} \backward{x}_0^i$, where
\begin{align}
    \backward{b}_{t}^i &= \sum_{j=1}^N \frac{\partial \normalized{w}_{t}^j}{\partial w_{t}^i} \backward{w}_{t}^j, \quad
    b_t^i = \sum_{j=1}^N \frac{\partial \normalized{w}_{t}^j}{\partial w_{t}^i} \frac{\partial}{\partial \normalized{w}_t^j} F_t(x_t^{1:N}, \normalized{w}_t^{1:N}, \theta) \\
    \backward{x}_t^i &= \sum_{j=1}^N \indicator_{a_t^j = i}
        \frac{\partial x_{t+1}^j}{\partial x_t^{a_t^j}} \left(
            \frac{\partial w_{t+1}^j}{\partial x_{t+1}^j} \hat{F}_{t+1} + W_{t+1} \left( \backward{x}_{t+1}^j
                +  \frac{\partial w_{t+1}^j}{\partial x_{t+1}^j} \backward{b}_{t+1}^j \right) \right) \\
    \backward{w}_t^i &= \sum_{j=1}^N \indicator_{a_t^j = i} \frac{N w_{t+1}^j}{\normalized{w}_t^i} \left( \hat{F}_{t+1} + W_{t+1} \backward{b}_{t+1}^j \right) \\
    \backward{\theta}_t &= \left( \backward{\theta}_{t+1} +
            \sum_{i=1}^N \frac{\partial x_{t+1}^i}{\partial \theta} \left( \backward{x}_{t+1}^j
                +  \frac{\partial w_{t+1}^i}{\partial x_{t+1}^i} \backward{b}_{t+1}^i \right) +
                \frac{\partial w_{t+1}^i}{\partial \theta} \backward{b}_{t+1}^i \right) W_{t+1} \\
        &+ \hat{F}_{t+1} \sum_{i=1}^N \left( \frac{\partial w_{t+1}}{\partial \theta} + \frac{\partial x_{t+1}^i}{\partial \theta} \frac{\partial w_{t+1}^i}{\partial x_{t+1}^i} \right)
\end{align}
for $0 \leq t < T$ and $\backward{x}_T^i = \backward{w}_T^i = \backward{\theta}_T = 0$ for all $i$.
\end{definition}
The overhead left arrow denotes backward messages, which constitute unbiased estimators for partial derivatives of $F_t$. We define $b_t^i$ and $\backward{b}_t^i$ solely to save space and avoid repetitions.

\begin{theorem} \label{th:unbiased}
The DPF-SGR gradient $G(\theta)$ from Definition \ref{def:gradients} is an unbiased estimator for the total derivative of the marginal likelihood $\frac{dZ}{d\theta}$.
\end{theorem}
\begin{proof}
The proof is by induction going backwards in time. The inductive hypothesis is that the backward messages from Definition \ref{def:gradients} are unbiased estimators for the partial derivatives of $F_t$. The base case is trivial, since $F_T = 1$ is constant and the backward messages are all zero. Then for the inductive step we have
\begin{align}
    &\frac{\partial}{\partial \normalized{w}_t^i} F_t(x_t^{1:N}, \normalized{w}_t^{1:N}, \theta) =
    \frac{\partial}{\partial \normalized{w}_t^i} \expect{F_t(x_t^{a_t^{1:N}}, \resampled{w}_t^{1:N}, \theta)}{a_t^i \sim R(r_t^{1:N})} = \\
    &\expect{\sum_{j=1}^N \frac{\partial \resampled{w}_t^j}{\partial \normalized{w}_t^i} \frac{\partial}{\partial \resampled{w}_t^j} F_t(x_t^{a_t^{1:N}}, \resampled{w}_t^{1:N}, \theta)}{a_t^i \sim R(r_t^{1:N})} = \\
    &\expect{\sum_{j=1}^N \indicator_{a_t^j = i} \frac{1}{r_t^i} \frac{\partial}{\partial \resampled{w}_t^j} \expect{W_{t+1} F_{t+1}(x_{t+1}^{1:N}, \normalized{w}_{t+1}^{1:N}, \theta)}{\epsilon_{t+1}^{1:N} \sim \mathcal{N}}}{a_t^i \sim R(r_t^{1:N})} = \\
    &\expect{\expect{\sum_{j=1}^N \indicator_{a_t^j = i} \frac{1}{r_t^i} \left( F_{t+1} \frac{\partial W_{t+1}}{\partial \resampled{w}_t^j} + W_{t+1} \frac{\partial}{\partial \resampled{w}_t^j} F_{t+1}(x_{t+1}^{1:N}, \normalized{w}_{t+1}^{1:N}, \theta) \right)}{\epsilon_{t+1}^{1:N} \sim \mathcal{N}}}{a_t^i \sim R(r_t^{1:N})} = \\
    &\expect{\expect{\sum_{j=1}^N \indicator_{a_t^j = i} \frac{1}{r_t^i} \frac{\partial w_{t+1}^j}{\partial \resampled{w}_t^j} \left( F_{t+1} + W_{t+1} b_{t+1}^j \right)}{\epsilon_{t+1}^{1:N} \sim \mathcal{N}}}{a_t^i \sim R(r_t^{1:N})} = \\
    &\expect{\expect{\expect{\sum_{j=1}^N \indicator_{a_t^j = i} \frac{N w_{t+1}^j}{\normalized{w}_t^i} \left( \hat{F}_{t+1} + W_{t+1} \backward{b}_{t+1}^j \right)}{PF}}{\epsilon_{t+1}^{1:N} \sim \mathcal{N}}}{a_t^i \sim R(r_t^{1:N})} = \\
    &\expect{\expect{\expect{\backward{w}_t^i}{PF}}{\epsilon_{t+1}^{1:N} \sim \mathcal{N}}}{a_t^i \sim R(r_t^{1:N})}
\end{align}
and similarly for partial derivatives with respect to $x_t^i$ and $\theta$, although the expressions involved are more complicated. In those equations we perform weighted resampling and then complete the proof of the inductive step by setting $r_t^i = \normalized{w}_t^i$. The crucial property that makes this proof work is that the terms involving $F_{t+1}$ or its derivatives only appear linearly, so in expectation we can replace them with the relevant backward messages. Finally, we use the law of total derivative, and the fact that the initial weights are uniform, to complete the proof of the theorem.
\begin{align}
    &\expect{G(\theta)}{PF} = \expect{\backward{\theta}_0 + \frac{1}{N} \sum_{i=1}^{N} \frac{d x_0^i}{d \theta} \backward{x}_0^i}{PF} = \\
    &\left( \frac{\partial}{\partial \theta} + \frac{1}{N} \sum_{i=1}^N \frac{dx_0^i}{d\theta} \frac{\partial}{\partial x_0^i} \right)
        F_0(x_0^{1:N}, w_0^{1:N}, \theta) =
    \frac{d}{d\theta} F_0(x_0^{1:N}, w_0^{1:N}, \theta) = \frac{dZ}{d\theta}
\end{align}
\end{proof}


% \subsection{Non-reparameterizable latent variables} \label{sec:latent-vars}

% While in Section \ref{sec:diff-resampling} we assumed that the proposal distributions used for the latent variables are reparameterizable, it is straightforward to extend DPF-SGR to the non-reparameterizable case. Specifically, we would sample $x_{t+1}^i$ directly from $q_{\theta}$ and the resulting weight would be
% \begin{align}
%     w_{t+1}^i = \resampled{w}_t^i \frac{p_{\theta}(x_{t+1}^i, y_{t+1} | x_t^{a_t^i})}{\stopgrad{q_{\theta}(x_{t+1}^i | x_t^{a_t^i}, y_{t+1})}} .
% \end{align}
% In other words, if the proposal distribution is not reparameterized, its density in the importance weight should have stop-gradient applied to it. Although we do not pursue this direction further in this paper, it is clear that the resulting gradient estimator would be unbiased, but it is not clear whether its variance would be low enough to make it practical.

% In the absence of resampling, or even any sequential structure, DPF-SGR reduces to normal importance sampling. When the reparameterization trick is used for the latent variables, this recovers the setting used in importance-weighted auto-encoders (IWAE) \citep{burda_importance_2016}. When they are not, however, we obtain a multi-sample objective different from IWAE with score function corrections, since the corrections now go inside the logarithm. We leave investigating this objective for future work.


==> sections/4_experiments.tex <==
\section{Experiments} \label{sec:experiments}

In this section we experimentally evaluate the performance of DPF-SGR. We use the following baselines: sequential importance sampling without resampling (SIS), biased particle filter ignoring the gradients resulting from resampling (PF), a particle filter with score function corrections (PF-SF), and the differentiable particle filter based on optimal transport of \cite{corenflos_differentiable_2021} (DPF-OT). We borrow the experimental setup from \citet{le_auto-encoding_2018} and \citet{corenflos_differentiable_2021}, using the code released with those papers with the modifications needed to implement DPF-SGR. Comparisons with DPF-OT are only available in Section \ref{sec:volatility}, since the remaining experiments use the code form \citet{le_auto-encoding_2018}, where DPF-OT is not available.

\subsection{Linear Gaussian State Space Model} \label{sec:lgssm}
In the first experiment we use a Linear Gaussian State Space Model (LGSSM) with a bootstrap proposal exactly as specified by \citet{le_auto-encoding_2018}, with two global parameters, a one dimensional latent variable and 200 time steps. Figure \ref{fig:experiments/lgssm} in our paper corresponds exactly to Figure 2 from \citet{le_auto-encoding_2018}, with DPF-SGR and PF-SF added. We find that using stop-gradient resampling offers a noticeable improvement over the standard PF in the low particle regime, while in the high particle regime DPF-SGR achieves faster convergence at the expense of a minimal decrease in the final performance, shown in Table \ref{tab:bouncing_ball}.

% We also use the LGSSM to quantitatively evaluate bias and variance of the gradient estimators produced by different methods. Figure \ref{fig:experiments/bias_variance}\todo{Remove legend on top plot} shows the results for both gradients of $Z$ and $\log Z$, evaluated for $\theta_1$ on a fixed sequence $y_{1:5}$. Unlike PF, DPF-SGR produces unbiased gradient estimates, with only a small increase in variance.\todo{Revise once final results are in.}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.9\textwidth]{sections/figs/bias_variance/logZ.pdf}
%     \includegraphics[width=0.9\textwidth]{sections/figs/bias_variance/Z.pdf}
%     \caption{Mean (left) and standard deviation (right) of the gradient estimators for $Z$ (bottom) and $log Z$ (top) obtained with different particle filter variants. For each point on the plot we used 10,000 independent runs of the particle filter. The ground truth value is computed using SIS with 1 million samples.}
%     \label{fig:experiments/bias_variance}
% \end{figure}

\subsection{Stochastic Volatility Model} \label{sec:volatility}

\begin{figure}[t]
    \centering
    % \includegraphics[width=0.32\textwidth]{sections/figs/stochastic_vol/loglik.pdf}
    \includegraphics[width=0.49\textwidth]{sections/figs/stochastic_vol/mu_diff.pdf}
    \includegraphics[width=0.49\textwidth]{sections/figs/stochastic_vol/wallclock.pdf}
    \caption{Left is the L1 error in parameter estimation throughout the training of the stochastic volatility model. With 10 particles the error in $\mu$ starts increasing towards the end of training, indicating overfitting. Right is the average wall clock execution time for a single forward and backward pass for each particle filter variant.}
    \label{fig:experiments/stochastic_volitility}
\end{figure}


In this experiment we learn the parameters of a stochastic volatility model, a popular financial model for which particle filters are known to perform well. We use the implementation provided in the code repository associated with the paper of \citet{corenflos_differentiable_2021}\footnote{\url{https://github.com/JTT94/filterflow}}, which allows us to reuse the DPF-OT settings provided by the original authors. The model is described by the following equations:
\begin{align}
x_0 &\sim \mathcal{N}\left(0, \frac{\sigma^2_x}{(1 -  \phi^2)}\right)\\
    x_{t+1} &= \mu\cdot(1 - \phi) + \phi\cdot x_t + \sigma_x \cdot \eta_t, & \eta_t &\sim \mathcal{N}(0,1), t = 1,..., T,\\
    y_t &= \epsilon_t \cdot  \exp\left(\frac{x_t}{2}\right), & \epsilon_t &\sim \mathcal{N}(0,1) .
\end{align}

We generate synthetic data with T = 100, $\mu$ = 2, $\phi$ = 0.9, $\sigma_x$ = 1, $\theta_{1:3} = \{\mu,\phi, \sigma_x \}$ and train the model for 500 epochs using Adam with a learning rate of $0.01$. Resampling is triggered when the effective sample size falls beneath $N/2$, and for all methods we use the bootstrap proposal like in the LGSSM experiment in Section \ref{sec:lgssm}. Figure \ref{fig:experiments/stochastic_volitility} shows progression of the parameter estimation error $|\hat{\mu} - \mu|$ throughout training and the execution time of different algorithms. DPF-SGR produces results at least on par with DPF-OT, while executing almost as fast as PF.
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.49\textwidth]{sections/figs/stochastic_vol/wallclock.pdf}
%     \caption{Average wall clock execution time for a single forward and backward pass for each particle filter variant. We average 10 runs and the error bars show the standard deviation of measurements. DPF-OT incurs a siginificant computational overhead, while DPF-SGR does not.}
%     \label{fig:experiments/stochastic_volitility_wallclock}
% \end{figure}


\subsection{Variational Recurrent Neural Network} \label{sec:agents}

In our final experiment we train a variational recurrent neural network (VRNN) modeling the movement of agents in a 2D world where the obvservations are provided in the form of partially occluded images. We use the setting introduced by \citet{le_auto-encoding_2018}, with 32x32 images and 40 time steps. In this experiment we train an inference network jointly with the model, as is typically done in VRNNs. Our Figure \ref{fig:experiments/bouncing_ball} corresponds exactly to Figure 4 of \citet{le_auto-encoding_2018}, except that we show performance both on the training and test sets. While PF achieves better performance on the training set, this is largely a result of overfitting, with DPF-SGR learning slower but ultimately achieving better test set performance. The numerical values for the best test set log-marginal likelihood for each method are shown in Table \ref{tab:bouncing_ball}.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.49\textwidth]{sections/figs/bouncing_ball/bouncing_ball_train.pdf}
    \includegraphics[width=0.49\textwidth]{sections/figs/bouncing_ball/bouncing_ball_test.pdf}
    \caption{Log-marginal likelihood estimates for training and test set throughout the training of the VRNN model. Unlike DPF-SGR, SIS and PF show clear signs of overfitting.}
    \label{fig:experiments/bouncing_ball}
\end{figure}



\begin{table}
    \centering
    \begin{tabular}{llr}
            \toprule
            N   &     Method   &  LGSSM \\
            \midrule
                  & PF-SF           &       -475.73 $\pm$ 55.69  \\
           10     & SIS             &       -2742.99 $\pm$ 279.97 \\
                  & PF              &       -300.46 $\pm$ 2.62 \\
                  & DPF-SGR (us)    &       \textbf{-292.70 $\pm$ 1.28} \\
            \midrule
                  &   PF-SF              &       -1038.85 $\pm$ 176.02\\
            10k   &   SIS                &       -343.65 $\pm$ 15.61\\
                  &   PF                 &       \textbf{-290.04 $\pm$ 0.00}\\
                  &   DPF-SGR (us)       &       -290.08 $\pm$ 0.02 \\
            \bottomrule
        \end{tabular}
    \quad
    \begin{tabular}{llr}
        \toprule
        N     &     Method   & VRNN \\
        \midrule
                & --   & \multicolumn{1}{c}{--} \\
         10     & SIS           &       -356.22 $\pm$ 0.08 \\
               & PF            &       -355.98 $\pm$ 0.13  \\
              & DPF-SGR (us)  &       \textbf{-355.82 $\pm$ 0.14} \\
        \midrule
                & -- &                  \multicolumn{1}{c}{--}        \\
        20    & SIS              &       -356.41 $\pm$ 0.50\\
              & PF               &       -355.97 $\pm$ 0.16\\
              & DPF-SGR (us)     &       \textbf{-355.74 $\pm$ 0.02} \\
        \bottomrule
    \end{tabular}
    \vspace{5mm}
    \caption{Best values for the test set log-marginal likelihood $\log Z$ for $N$ particles in the LGSSM/VRNN experiments in \cref{fig:experiments/lgssm} and \cref{fig:experiments/bouncing_ball} respectively. }
    \label{tab:bouncing_ball}
    \end{table}

% \begin{table}
% \centering
% \begin{tabular}{llr}
%         \toprule
%         N   &     Method   &  LGSSM \\
%         \midrule
%               & SIS             &       -2742.99 $\pm$ 279.97 \\
%          10     & PF              &       -300.46 $\pm$ 2.62 \\
%             & PF-SF           &       -475.73 $\pm$ 55.69  \\
%               & DPF-SGR (us)    &       \textbf{-292.70 $\pm$ 1.28} \\
%         \midrule
%           &   SIS                &       -343.65 $\pm$ 15.61\\
%       10k    &   PF                 &       \textbf{-290.04 $\pm$ 0.00}\\
%         &   PF-SF              &       -1038.85 $\pm$ 176.02\\
%           &   DPF-SGR (us)       &       -290.08 $\pm$ 0.02 \\
%         \bottomrule
%     \end{tabular}
% \quad
% \begin{tabular}{llr}
%     \toprule
%     N   &     Method   & VRNN \\
%     \midrule
%           & SIS           &       -356.22 $\pm$ 0.08 \\
%      10   & PF            &       -355.98 $\pm$ 0.13  \\
%         \\
%           & DPF-SGR (us)  &       \textbf{-355.82 $\pm$ 0.14} \\
%     \midrule
%       & SIS              &       -356.41 $\pm$ 0.50\\
%   20  & PF               &       -355.97 $\pm$ 0.16\\
%   \\
%       & DPF-SGR (us)     &       \textbf{-355.74 $\pm$ 0.02} \\
%     \bottomrule
% \end{tabular}
% \vspace{5mm}
% \caption{Best values for the test set log-marginal likelihood $\log Z$ for $N$ particles in the LGSSM/VRNN experiments in \cref{fig:experiments/lgssm} and \cref{fig:experiments/bouncing_ball} respectively. }
% \label{tab:bouncing_ball}
% \end{table}


==> sections/5_conclusion.tex <==
\section{Discussion} \label{sec:discussion}

The algorithm we developed in this work, DPF-SGR, provides unbiased gradients of marginal likelihood $\grad Z$ using a standard forward pass of a particle filter and a non-standard backward pass. It is worth noting that in most applications, including the experiments in this paper, we optimize in the log space, estimating $\grad \log Z$ instead. While in practice we can simply apply automatic differentiation to $\log \hat{Z}$ and use gradient-based optimization, technically the gradients obtained in this fashion are biased estimators of $\grad \log Z$, both for DPF-SGR and all the other variants of particle filters considered in this paper. This is because even on the forward pass, the particle filter does not provide unbiased estimates of $\log Z$.

The estimators for $\grad \log Z$ produced by PF-SF can be regarded as unbiased estimators for a gradient of a lower bound to $\log Z$ \citep{le_auto-encoding_2018}, similarly to the ELBO objective used in VAEs. This is not necessarily the case for the biased PF ignoring resampling gradients. DPF-OT produces unbiased gradient estimates for some objective, but it is not necessarily a lower bound to $\log Z$, since the estimator for $Z$ produced by DPF-OT on the forward pass is itself biased. DPF-SGR can be regarded as making the following approximation
\begin{align*}
    \grad \log Z = \grad \log \expect{\hat{Z}}{PF} = \frac{\grad \expect{\hat{Z}}{PF}}{\expect{\hat{Z}}{PF}}
    = \frac{\expect{\grad \hat{Z}}{PF}}{\expect{\hat{Z}}{PF}}
    \approx \expect{\frac{\grad \hat{Z}}{\hat{Z}}}{PF} = \expect{\grad \log \hat{Z}}{PF} ,
\end{align*}
where the differentiable property of DFT-SGR lets us push the gradient inside the expectation. Just like with PF, the resulting gradients do not necessarily correspond to any particular objective, but in practice we find this does not cause problems with optimization. Unlike for PF, we expect the estimator for $\grad \log Z$ produced by DPF-SGR to be consistent in most circumstances, although establishing the precise conditions for that is an important direction for future work.

In this paper we have treated the stop-gradient operator somewhat informally, following \citet{foerster_dice_2018}, using it as a normal function even though no function with the required properties exists.  A formal definition would potentially allow us to make the arguments we make in Section \ref{sec:sgr} rigorous, avoiding the construction we use in Section \ref{sec:theory} entirely. This is likely to involve significant effort, since it requires opening the black box of automatic differentiation.

Finally, it is natural to ask how DPF-SGR relates to PF-SF, since the two coincide when only a single particle is used. Intuitively, we can think of DPF-SGR as performing additional cancellations of the score function terms, beyond what would be possible with independence analysis only \citep{schulman_gradient_2016}, since due to resampling steps all future variables depend an all current weights. The precise nature of those cancellations is difficult to characterize, but perhaps further investigation can explain why DPF-SGR achieves good performance without additional variance reduction steps and maybe suggest additional improvements.

==> sections/app/app.tex <==
\section{Appendix}


==> sections/checklist.tex <==
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{In Section \ref{sec:discussion} we point out that our method only produces unbiased gradients for $Z$ and not $\log Z$. We also point out the informal nature of the stop-gradient estimator.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{The proposed algorithm is very general without ties to particular applications.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{The technical assumptions are stated in Section \ref{sec:pf}.}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{Full proof of Theorem \ref{th:unbiased} included in main text.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Yes code will be made publicly available at \url{https://github.com/vmasrani/stopgrad_pf}}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Yes}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{Yes}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Code was run on an internal cluster and we benchmark our method against sota baseline in terms of wallclock time in main text.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Yes we use two code repositories and credit the creators in main text}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}
